The LAMBADA dataset: Word prediction requiring a broad discourse context

We introduce LAMBADA, a dataset to evaluate the capabilities of computational models for text understanding by means of a word prediction task. LAMBADA is a collection of narrative passages sharing the characteristic that human subjects are able to guess their last word if they are exposed to the whole passage, but not if they only see the last sentence preceding the target word. To succeed on LAMBADA, computational models cannot simply rely on local context, but must be able to keep track of information in the broader discourse. We show that LAMBADA exemplifies a wide range of linguistic phenomena, and that none of several state-of-the-art language models reaches accuracy above 1% on this novel benchmark. We thus propose LAMBADA as a challenging test set, meant to encourage the development of new models capable of genuine understanding of broad context in natural language text.

==> old-table-examples.tex <==
%%%% TABLE WITH EXAMPLES %%%%

\setcounter{ExNo}{0}

\begin{figure*}[p] \small \centering
\hrule

\

\ex. \label{ex:miscarriage}
\begin{description}[nolistsep]
\item[{\rm \em Context:}] ~``Yes, I thought I was going to lose the baby.''   ``I was scared too,''
 he stated, sincerity flooding his eyes.   ``You were ?''  ``Yes, of
 course.   Why do you even ask?''  ``This baby wasn't exactly planned
 for.''
 \item[\rm \em Target sentence:]~ ``Do you honestly think that I would want you to have a \_\_\_\_\_ ?''
 \item[\rm \em Target word:]~ miscarriage %noun not in the context, the
                                %scene need to be understood.
\end{description}


\ex.  \label{ex:Gabriel}
\begin{description}[nolistsep]
\item[{\rm \em Context:}]~ ``Why?"   ``I would have thought you'd find him rather dry," she said.   ``I don't know about that," said Gabriel.   ``He was a great craftsman," said Heather.   ``That he was," said Flannery. 
\item[\rm \em Target sentence:]~  ``And Polish, to boot," said \_\_\_\_\_. 
\item[\rm \em Target word:]~Gabriel %NNP in context -- several NNPs in
                                %passage; passage dialouge
\end{description}

%%Examples with Target_Verbs (not in context.)
%%\begin{description}[nolistsep]  
%%\item[{\rm \em Context:}] That made a million questions tear through his mind-almost made him stop running.   Mistress Jane.   He couldn't possibly accept that she was on his side.   "Sato!"   He looked down to see Tick's face in the water, his hand reaching out for him. 
%%\item[\rm \em Target sentence:]  He was still thrashing as if he might \_\_\_\_\_. 
%%\item[\rm \em Target word:] drwon
%%\end{description}\\[-5pt]
%%\hline

\ex. \label{ex:intervene}
\begin{description}[nolistsep]
\item[{\rm \em Context:}] As I guzzled my sports drink, I noticed a figure dressed in all-black stealthily creep up to an SUV in the parking lot of the 24-hour pharmacy.   What do we have here?   I wondered as he started to fidget with the driver's side door of the vehicle.   It took me a few moments to realize that the man was breaking into the SUV.
\item[\rm \em Target sentence:]  Having just committed a burglary of my own across town, I felt no need to \_\_\_\_\_.
\item[\rm \em Target word:] intervene
\end{description}

\ex. \label{ex:coffee}
\begin{description}[nolistsep]
\item[{\rm \em Context:}]~Both its sun-speckled shade and the cool grass beneath were a welcome
respite after the stifling kitchen, and I was glad to relax against
the tree's rough, brittle bark and begin my breakfast of buttery,
toasted bread and fresh fruit.   Even the water was tasty, it was so clean and cold. 
\item[\rm \em Target sentence:] ~ It almost made up for the lack of  \_\_\_\_\_.  
\item[\rm \em Target word:] ~coffee
\end{description}


\ex. \label{ex:driving}
\begin{description}[nolistsep]
\item[{\rm \em Context:}] ~ The battery on Logan's radio must have been on the way out.   So he told himself.   There was no other explanation beyond Cygan and the staff at the White House having been overrun.   Lizzie opened her eyes with a flutter.   They had been on the icy road for an hour without incident. 
\item[\rm \em Target sentence:] ~ Jack was happy to do all of the \_\_\_\_\_.  
\item[\rm \em Target word:]~ driving 
\end{description}

\ex. \label{ex:died}
\begin{description}[nolistsep] 
\item[{\rm \em Context:}]~  ``Again, he left that up to you.   However, he was adamant in his
 desire that it remain a private ceremony.   He asked me to make sure,
 for instance, that no information be given to the newspaper regarding
 his death, not even an obituary.
\item[\rm \em Target sentence:] ~   
  I got the sense that he didn't want anyone, aside from the three of
 us, to know that he'd even \_\_\_\_\_.
\item[\rm \em Target word:]~ died % 'death' (nominal form of the verb) in the context 
\end{description}

%%\hline\begin{description}[nolistsep]
%%\item[{\rm \em Context:}]  The gift she'd gotten him, which was sitting in her bag, seemed silly now.   She couldn't accept a house from him.   She could live there as long as they were married, but when the fairytale ended, she couldn't keep the place. 
%%\item[\rm \em Target sentence:]  She was still overwhelmed and
%%thrilled he would do something so \_\_\_\_\_.
%%\item[\rm \em Target word:] generous 
%%\end{description}\\
%%\hline\begin{description}[nolistsep]  
%%\item[{\rm \em Context:}] Michelle guided Danny and me into Aunt Polly's room.   Michelle's parents and Aunt Jessy gathered too.   All the tubes and wires were gone.   This looked better, and I think she must have liked it that way, because her eyes still shined like they had the last time we'd seen her. 
%%\item[\rm \em Target sentence:]  The rest of her was a wrinkled gray sheet, but her eyes were  \_\_\_\_\_.  
%%\item[\rm \em Target word:] brilliant
%%\end{description}\\
%%Target JJ
%%\hline\begin{description}[nolistsep]
%%\item[{\rm \em Context:}] He picked her up, walked to the bedroom door, and slowly pulled it
%%open.   The hallway was dark, quiet.   He crept down it, heard
%%Rachael's mother snoring in the guest room.   Rachael's sister, Elise,
%%was asleep on the sofa in the den. 
%%\item[\rm \em Target sentence:]  The creak of the front door opening made her shift, but she didn't \_\_\_\_\_. 
%%\item[\rm \em Target word:] wake
%%\end{description}\\
%
%% GBT: commenting it out on purpose -- too difficult and also this
%% category is over-represented in the table
%% \hline
%% (5) & 
%% \begin{description}[nolistsep]
%% \item[{\rm \em Context:}]  All of our arenas are most probably throwbacks to that earlier era, although the activities in modern centers are tamed down somewhat from the bloodthirsty times gone past... at least, a little bit.   After learning about a game known as ` Bull Poker ', though, I have my doubts.   Four men sit at a poker table, ostensibly playing cards, as an angry bull is released into the ring. 
%% \item[\rm \em Target sentence:]  Apparently, the last one at the table \_\_\_\_\_. 
%% \item[\rm \em Target word:]  wins %to guess the verbs, the scene has
%%                                 %to be understood. 
%% \end{description}\\[-5pt]
%%\hline\begin{description}[nolistsep]
%%\item[{\rm \em Context:}]  My assessment of being dead before lunch wasn't too far off base.   Irritably, Ezra shook his head, stalking toward "our" mat.   "What kind of training have you had ?"   I gulped, and hurried to catch up.   "Uh, none." 
%%\item[\rm \em Target sentence:]  "Perfect," he muttered, facing me on the \_\_\_\_\_. 
%%\item[\rm \em Target word:] mat
%%\end{description}\\
%\hline

\ex. \label{ex:chains} 
\begin{description}[nolistsep]
\item[{\rm \em Context:}]~  Preston had been the last person to wear those chains, and I knew what I'd see and feel if they were slipped onto my skin-the Reaper's unending hatred of me.   I'd felt enough of that emotion already in the amphitheater.   I didn't want to feel anymore.   ``Don't put those on me," I whispered.   ``Please." 
\item[\rm \em Target sentence:]~  Sergei looked at me, surprised by my low, raspy please, but he put down the \_\_\_\_\_.  
\item[\rm \em Target word:]~ chains %noun in the context, at the
                                %beginning of the passage.
\end{description}

%%\hline\begin{description}[nolistsep]
%%\item[{\rm \em Context:}]  Recall our encounter with the warbirds at the Federation border.   Confirm my memory with yours."   She turned Seren to face her.   They placed their foreheads together as when they meditated together.   They held hands beneath the surface of the water.   They closed their eyes. 
%%\item[\rm \em Target sentence:]  "There were five warbirds at the \_\_\_\_\_." 
%%\item[\rm \em Target word:] border
%%\end{description}\\
%%\hline
%%Verbs in context
%%\hline\begin{description}[nolistsep] 
%% \item[{\rm \em Context:}]  "If you wanted me to have a happy birthday, you'd come over to my
%% party."   "Your party," I repeated flatly.   "Yeah, remember ?
%% Andrea invited you ?"   I remembered.   I'd been thinking about it
%% every day this week. 
%%\item[\rm \em Target sentence:]  "I didn't think I was still \_\_\_\_\_." 
%%\item[\rm \em Target word:] invited
%%\end{description}\\
%\hline

\ex. \label{ex:dancing} 
\begin{description}[nolistsep]
\item[{\rm \em Context:}]~  They tuned, discussed for a moment, then struck up a lively jig.   Everyone joined in, turning the courtyard into an even more chaotic scene, people now dancing in circles, swinging and spinning in circles, everyone making up their own dance steps.   I felt my feet tapping, my body wanting to move. 
\item[\rm \em Target sentence:] ~ Aside from writing, I 've always loved \_\_\_\_\_.  
\item[\rm \em Target word:]~ dancing
\end{description}

\ex. \label{ex:lonely}
\begin{description}[nolistsep] 
\item[{\rm \em Context:}]~  My wife refused to allow me to come to Hong Kong when the plague was at its height and --" ``Your wife, Johanne?   You are married at last ?"   Johanne grinned.   ``Well, when a man gets to my age, he starts to need a few home comforts. 
\item[\rm \em Target sentence:] ~   After my dear mother passed away
  ten years ago now, I became \_\_\_\_\_.
\item[\rm \em Target word:]~ lonely
\end{description}

%% GBT: I would not put 2 Lambada examples of adjectives, it'd be greatly over-represented...
%% \hline
%% (11) & 
%% \begin{description}[nolistsep] 
%% \item[{\rm \em Context:}]   He was almost ashamed to admit it, but there was something about her that scared him a little.   Ann peeked her head through the first curtain.   "Nope."   Mike looked in after her, to find an older woman asleep.   He quickly closed up the curtain.   "Ann, we can't just disturb these patients until we find your doctor. 
%% \item[\rm \em Target sentence:]    Don't you think it's a little \_\_\_\_\_?" 
%% \item[\rm \em Target word:] rude 
%% \end{description}\\
%%\hline\begin{description}[nolistsep] 
%%\item[{\rm \em Context:}]  
%%\item[\rm \em Target sentence:]    
%%\item[\rm \em Target word:] 
%%\end{description}\\
%\hline

\hrule
  \caption{Examples of LAMBADA passages.}
  \label{fig:examples-lambada}
\end{figure*}

\setcounter{ExNo}{1}
%%% END OF TABLE WITH EXAMPLES %%%%

% previous figure

%\begin{figure*}[htb] \small
%  \centering
%  \begin{tabular}{|p{15cm}|}  \hline
%    \emph{Context:} As I guzzled my sports drink, I noticed a figure dressed in all-black stealthily creep up to an SUV in the parking lot of the 24-hour pharmacy.   What do we have here?   I wondered as he started to fidget with the driver's side door of the vehicle.   It took me a few moments to realize that the man was breaking into the SUV.\\
%    \emph{Target sentence:}  Having just committed a burglary of my own across town, I felt no need to \_\_\_\_\_.\\
%    \emph{Target word:} intervene\\
%    \hline
%  \end{tabular}
%  \caption{One Lambada datapoint (passage).}
%  \label{fig:examples-lambada}
%\end{figure*}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:



%%%%% TABLE WITH EXAMPLES %%%%
%
%\begin{figure*}[t] \small \centering
%\begin{tabular}{|cp{14.5cm}|}  \hline
%% (1) & 
%% \begin{description}[nolistsep]
%% \item[{\rm \em Context:}]  She knew that Basha was a decent young man, that he was pretty sweet and friendly with her.   Jawen knew they had a bit of a history, but she thought that this time she would get along better with him, that she could overlook those problems.   They kissed, and she knew that she liked Basha, but then Hastin interfered.  
%% \item[\rm \em Target sentence:]  She was so angry that she immediately
%%   said, once they were out of earshot of Basha, "You don't mean
%%   anything to me anymore, \_\_\_\_\_ . 
%% \item[\rm \em Target word:] Hastin %NNP in context -- several NNPs in
%%                                 %passage, passage discourses
%%\end{description}\\[-5pt]
%%\hline
%(1) & 
%\begin{description}[nolistsep]
%\item[{\rm \em Context:}] ``Yes, I thought I was going to lose the baby.''   ``I was scared too,''
% he stated, sincerity flooding his eyes.   ``You were ?''  ``Yes, of
% course.   Why do you even ask ?''  ``This baby wasn't exactly planned
% for.''
% \item[\rm \em Target sentence:]  ``Do you honestly think that I would want you to have a \_\_\_\_\_ ?''
% \item[\rm \em Target word:] miscarriage %noun not in the context, the
%                                %scene need to be understood.
%\end{description}\\[-5pt]
%\hline
%(2) & 
%\begin{description}[nolistsep]
%\item[{\rm \em Context:}]  "Why ?"   "I would have thought you'd find him rather dry," she said.   "I don't know about that," said Gabriel.   "He was a great craftsman," said Heather.   "That he was," said Flannery. 
%\item[\rm \em Target sentence:]  "And Polish, to boot," said \_\_\_\_\_. 
%\item[\rm \em Target word:] Gabriel %NNP in context -- several NNPs in
%                                %passage; passage dialouge
%\end{description}\\[-5pt]
%\hline
%%Examples with Target_Verbs (not in context.)
%%\begin{description}[nolistsep]  
%%\item[{\rm \em Context:}] That made a million questions tear through his mind-almost made him stop running.   Mistress Jane.   He couldn't possibly accept that she was on his side.   "Sato!"   He looked down to see Tick's face in the water, his hand reaching out for him. 
%%\item[\rm \em Target sentence:]  He was still thrashing as if he might \_\_\_\_\_. 
%%\item[\rm \em Target word:] drwon
%%\end{description}\\[-5pt]
%%\hline
%(3) & 
%\begin{description}[nolistsep]
%\item[{\rm \em Context:}] As I guzzled my sports drink, I noticed a figure dressed in all-black stealthily creep up to an SUV in the parking lot of the 24-hour pharmacy.   What do we have here?   I wondered as he started to fidget with the driver's side door of the vehicle.   It took me a few moments to realize that the man was breaking into the SUV.
%\item[\rm \em Target sentence:]  Having just committed a burglary of my own across town, I felt no need to \_\_\_\_\_.
%\item[\rm \em Target word:] intervene
%\end{description}\\[-5pt]
%\hline
%(4) & 
%\begin{description}[nolistsep]
%\item[{\rm \em Context:}]  The battery on Logan's radio must have been on the way out.   So he told himself.   There was no other explanation beyond Cygan and the staff at the White House having been overrun.   Lizzie opened her eyes with a flutter.   They had been on the icy road for an hour without incident. 
%\item[\rm \em Target sentence:]  Jack was happy to do all of the \_\_\_\_\_.  
%\item[\rm \em Target word:] driving 
%\end{description}\\[-5pt]
%\hline
%(9) & 
%\begin{description}[nolistsep] 
%\item[{\rm \em Context:}]  ``Again, he left that up to you.   However, he was adamant in his
% desire that it remain a private ceremony.   He asked me to make sure,
% for instance, that no information be given to the newspaper regarding
% his death, not even an obituary.
%\item[\rm \em Target sentence:]    
%  I got the sense that he didn't want anyone, aside from the three of
% us, to know that he'd even \_\_\_\_\_.
%\item[\rm \em Target word:] died % 'death' (nominal form of the verb) in the context 
%\end{description}\\[-5pt]
%%\hline\begin{description}[nolistsep]
%%\item[{\rm \em Context:}]  The gift she'd gotten him, which was sitting in her bag, seemed silly now.   She couldn't accept a house from him.   She could live there as long as they were married, but when the fairytale ended, she couldn't keep the place. 
%%\item[\rm \em Target sentence:]  She was still overwhelmed and
%%thrilled he would do something so \_\_\_\_\_.
%%\item[\rm \em Target word:] generous 
%%\end{description}\\
%%\hline\begin{description}[nolistsep]  
%%\item[{\rm \em Context:}] Michelle guided Danny and me into Aunt Polly's room.   Michelle's parents and Aunt Jessy gathered too.   All the tubes and wires were gone.   This looked better, and I think she must have liked it that way, because her eyes still shined like they had the last time we'd seen her. 
%%\item[\rm \em Target sentence:]  The rest of her was a wrinkled gray sheet, but her eyes were  \_\_\_\_\_.  
%%\item[\rm \em Target word:] brilliant
%%\end{description}\\
%%Target JJ
%%\hline\begin{description}[nolistsep]
%%\item[{\rm \em Context:}] He picked her up, walked to the bedroom door, and slowly pulled it
%%open.   The hallway was dark, quiet.   He crept down it, heard
%%Rachael's mother snoring in the guest room.   Rachael's sister, Elise,
%%was asleep on the sofa in the den. 
%%\item[\rm \em Target sentence:]  The creak of the front door opening made her shift, but she didn't \_\_\_\_\_. 
%%\item[\rm \em Target word:] wake
%%\end{description}\\
%
%% GBT: commenting it out on purpose -- too difficult and also this
%% category is over-represented in the table
%% \hline
%% (5) & 
%% \begin{description}[nolistsep]
%% \item[{\rm \em Context:}]  All of our arenas are most probably throwbacks to that earlier era, although the activities in modern centers are tamed down somewhat from the bloodthirsty times gone past... at least, a little bit.   After learning about a game known as ` Bull Poker ', though, I have my doubts.   Four men sit at a poker table, ostensibly playing cards, as an angry bull is released into the ring. 
%% \item[\rm \em Target sentence:]  Apparently, the last one at the table \_\_\_\_\_. 
%% \item[\rm \em Target word:]  wins %to guess the verbs, the scene has
%%                                 %to be understood. 
%% \end{description}\\[-5pt]
%%\hline\begin{description}[nolistsep]
%%\item[{\rm \em Context:}]  My assessment of being dead before lunch wasn't too far off base.   Irritably, Ezra shook his head, stalking toward "our" mat.   "What kind of training have you had ?"   I gulped, and hurried to catch up.   "Uh, none." 
%%\item[\rm \em Target sentence:]  "Perfect," he muttered, facing me on the \_\_\_\_\_. 
%%\item[\rm \em Target word:] mat
%%\end{description}\\
%\hline
%(7) & 
%\begin{description}[nolistsep]
%\item[{\rm \em Context:}]  Preston had been the last person to wear those chains, and I knew what I'd see and feel if they were slipped onto my skin-the Reaper's unending hatred of me.   I'd felt enough of that emotion already in the amphitheater.   I didn't want to feel anymore.   "Don't put those on me," I whispered.   "Please." 
%\item[\rm \em Target sentence:]  Sergei looked at me, surprised by my low, raspy please, but he put down the \_\_\_\_\_.  
%\item[\rm \em Target word:] chains %noun in the context, at the
%                                %beginning of the passage.
%\end{description}\\[-5pt]
%%\hline\begin{description}[nolistsep]
%%\item[{\rm \em Context:}]  Recall our encounter with the warbirds at the Federation border.   Confirm my memory with yours."   She turned Seren to face her.   They placed their foreheads together as when they meditated together.   They held hands beneath the surface of the water.   They closed their eyes. 
%%\item[\rm \em Target sentence:]  "There were five warbirds at the \_\_\_\_\_." 
%%\item[\rm \em Target word:] border
%%\end{description}\\
%%\hline
%%Verbs in context
%%\hline\begin{description}[nolistsep] 
%% \item[{\rm \em Context:}]  "If you wanted me to have a happy birthday, you'd come over to my
%% party."   "Your party," I repeated flatly.   "Yeah, remember ?
%% Andrea invited you ?"   I remembered.   I'd been thinking about it
%% every day this week. 
%%\item[\rm \em Target sentence:]  "I didn't think I was still \_\_\_\_\_." 
%%\item[\rm \em Target word:] invited
%%\end{description}\\
%\hline
%(8) & 
%\begin{description}[nolistsep]
%\item[{\rm \em Context:}]  They tuned, discussed for a moment, then struck up a lively jig.   Everyone joined in, turning the courtyard into an even more chaotic scene, people now dancing in circles, swinging and spinning in circles, everyone making up their own dance steps.   I felt my feet tapping, my body wanting to move. 
%\item[\rm \em Target sentence:]  Aside from writing, I 've always loved \_\_\_\_\_.  
%\item[\rm \em Target word:] dancing
%\end{description}\\[-5pt]
%\hline
%(10) & 
%\begin{description}[nolistsep] 
%\item[{\rm \em Context:}]  My wife refused to allow me to come to Hong Kong when the plague was at its height and --" "Your wife, Johanne ?   You are married at last ?"   Johanne grinned.   "Well, when a man gets to my age, he starts to need a few home comforts. 
%\item[\rm \em Target sentence:]    After my dear mother passed away
%  ten years ago now, I became \_\_\_\_\_.
%\item[\rm \em Target word:] lonely
%\end{description}\\[-5pt]
%% GBT: I would not put 2 Lambada examples of adjectives, it'd be greatly over-represented...
%% \hline
%% (11) & 
%% \begin{description}[nolistsep] 
%% \item[{\rm \em Context:}]   He was almost ashamed to admit it, but there was something about her that scared him a little.   Ann peeked her head through the first curtain.   "Nope."   Mike looked in after her, to find an older woman asleep.   He quickly closed up the curtain.   "Ann, we can't just disturb these patients until we find your doctor. 
%% \item[\rm \em Target sentence:]    Don't you think it's a little \_\_\_\_\_?" 
%% \item[\rm \em Target word:] rude 
%% \end{description}\\
%%\hline\begin{description}[nolistsep] 
%%\item[{\rm \em Context:}]  
%%\item[\rm \em Target sentence:]    
%%\item[\rm \em Target word:] 
%%\end{description}\\
%\hline
%  \end{tabular}
%  \caption{Examples of LAMBADA passages.}
%  \label{fig:examples-lambada}
%\end{figure*}
%%%% END OF TABLE WITH EXAMPLES %%%%
%
%% previous figure
%
%%\begin{figure*}[htb] \small
%%  \centering
%%  \begin{tabular}{|p{15cm}|}  \hline
%%    \emph{Context:} As I guzzled my sports drink, I noticed a figure dressed in all-black stealthily creep up to an SUV in the parking lot of the 24-hour pharmacy.   What do we have here?   I wondered as he started to fidget with the driver's side door of the vehicle.   It took me a few moments to realize that the man was breaking into the SUV.\\
%%    \emph{Target sentence:}  Having just committed a burglary of my own across town, I felt no need to \_\_\_\_\_.\\
%%    \emph{Target word:} intervene\\
%%    \hline
%%  \end{tabular}
%%  \caption{One Lambada datapoint (passage).}
%%  \label{fig:examples-lambada}
%%\end{figure*}
%
%
%%%% Local Variables:
%%%% mode: latex
%%%% TeX-master: "main"
%%%% End:

